Adjoint-based optimal actuation for separated flow past an airfoil

This study computes the optimal normal actuation on the surface of a NACA0012 airfoil at an angle of attack of 15{\deg} and a Reynolds number of Re = 1000, using costs defined for minimal drag and maximal lift. To allow for a general actuation profile, non-zero actuation is permissible on both the suction and pressure surfaces. This approach of optimal actuation along the full airfoil surface augments most other studies that have focused on parametrically varied open-loop control restricted to the suction surface. The gradient-based optimization procedure requires the gradient of the cost functional with respect to the design variables, which is determined using the adjoint of the governing equations. The optimal actuation profile for the two performance aims are compared. Where possible, similarities with commonly considered open-loop actuation in the form of backward traveling waves on the suction surface have been highlighted. In addition, the key spatial locations on the airfoil surface for the two optimal control strategies have been compared to earlier works where actuation has been limited to a sub-domain of the airfoil surface. The flow features emerging from the optimal actuation variations, and their consequent influence on the instantaneous aerodynamic coefficients, have been analyzed. To complement our findings with normal actuation, we also provide in the appendix: results for a more general form of actuation with independent x and y components, and for a different optimization window to assess the effect of this window parameter on the actuation profile and the flow features.

==> References.tex <==
% This is jfm2esam.bib v1.0 08/14/02
%

%---Introduction
@article{seifert1996delay,
  title={Delay of airfoil stall by periodic excitation},
  author={Seifert, Avraham and Darabi, A and Wyganski, Israel},
  journal={Journal of aircraft},
  volume={33},
  number={4},
  pages={691--698},
  year={1996}
}

@article{amitay2002role,
  title={Role of actuation frequency in controlled flow reattachment over a stalled airfoil},
  author={Amitay, Michael and Glezer, Ari},
  journal={AIAA journal},
  volume={40},
  number={2},
  pages={209--216},
  year={2002}
}

@article{benard2009lift,
  title={Lift and drag performances of an axisymmetric airfoil controlled by plasma actuator},
  author={B{\'e}nard, Nicolas and Jolibois, J and Moreau, E},
  journal={Journal of Electrostatics},
  volume={67},
  number={2-3},
  pages={133--139},
  year={2009},
  publisher={Elsevier}
}


@article{chapin2015active,
  title={Active control of a stalled airfoil through steady or unsteady actuation jets},
  author={Chapin, VG and B{\'e}nard, Emmanuel},
  journal={Journal of Fluids Engineering},
  volume={137},
  number={9},
  pages={091103},
  year={2015},
  publisher={American Society of Mechanical Engineers}
}

@inproceedings{corke2002application,
  title={Application of weakly-ionized plasmas as wing flow-control devices},
  author={Corke, Thomas and Jumper, Eric and Post, Martiqua and Orlov, Dmitriy and McLaughlin, Thomas},
  booktitle={40th AIAA Aerospace Sciences Meeting \& Exhibit},
  pages={350},
  year={2002}
}

@ARTICLE{Corke2007,
	Author = {Corke, Thomas C and Post, Martiqua L and Orlov, Dmitry M},
	Date-Added = {2019-05-24 13:49:30 -0500},
	Date-Modified = {2019-05-24 13:49:30 -0500},
	Journal = {Progress in Aerospace Sciences},
	Number = {7-8},
	Pages = {193--217},
	Publisher = {Elsevier},
	Title = {{SDBD} plasma enhanced aerodynamics: concepts, optimization and applications},
	Volume = {43},
	Year = {2007}}

@ARTICLE{Corke2010,
	Author = {Corke, Thomas C and Enloe, C Lon and Wilkinson, Stephen P},
	Date-Added = {2019-05-24 13:49:30 -0500},
	Date-Modified = {2019-05-24 13:49:30 -0500},
	Journal = {Annual Review of Fluid Mechanics},
	Pages = {505--529},
	Publisher = {Annual Reviews},
	Title = {Dielectric barrier discharge plasma actuators for flow control},
	Volume = {42},
	Year = {2010}}

@inproceedings{Cutler2005,
	Author = {Cutler, Andrew and Beck, B and Wilkes, Jennifer and Drummond, J and Alderfer, David and Danehy, Paul},
	Booktitle = {43rd AIAA Aerospace Sciences Meeting and Exhibit},
	Date-Added = {2019-05-24 13:49:30 -0500},
	Date-Modified = {2019-05-24 13:49:30 -0500},
	Title = {Development of a pulsed combustion actuator for high-speed flow control},
	Year = {2005}}

@misc{Glezer2003,
	Author = {Glezer, Ari and Crittenden, Thomas M},
	Date-Added = {2019-05-24 13:49:30 -0500},
	Date-Modified = {2019-05-24 13:49:30 -0500},
	Month = apr # {~29},
	Note = {{U}S Patent 6,554,607},
	Publisher = {Google Patents},
	Title = {Combustion-driven jet actuator},
	Year = {2003}}
	
@ARTICLE{Crittenden2009,
	Author = {Crittenden, Thomas M and Raghu, Surya},
	Date-Added = {2019-05-24 13:49:30 -0500},
	Date-Modified = {2019-05-24 13:49:30 -0500},
	Journal = {International Journal of Flow Control},
	Number = {1},
	Pages = {87--97},
	Publisher = {Multi-Science Publishing Co. Ltd., 5 Wates Way Brentwood Essex CM 15 9 TB~{\ldots}},
	Title = {Combustion powered actuator with integrated high frequency oscillator},
	Volume = {1},
	Year = {2009}}




%*---Introduction:Findings
@article{chang1992forcing,
  title={Forcing level effects of internal acoustic excitation on the improvement of airfoil performance},
  author={Chang, RC and Hsiao, F-B and Shyu, R-N},
  journal={Journal of Aircraft},
  volume={29},
  number={5},
  pages={823--829},
  year={1992}
}

@article{hsiao1990control,
  title={Control of wall-separated flow by internal acoustic excitation},
  author={Hsiao, Fei-Bin and Liu, Chin-Fung and Shyu, Jong-Yaw},
  journal={AIAA journal},
  volume={28},
  number={8},
  pages={1440--1446},
  year={1990}
}

@ARTICLE{raju2008dynamics,
  title={Dynamics of airfoil separation control using zero-net mass-flux forcing},
  author={Raju, Reni and Mittal, Rajat and Cattafesta, Louis},
  journal={AIAA Journal},
  volume={46},
  number={12},
  pages={3103--3115},
  year={2008}
}

@inproceedings{kotapati2007numerical,
  title={Numerical simulations of synthetic jet based separation control in a canonical separated flow},
  author={Kotapati, Rupesh and Mittal, Rajat and Marxen, Olaf and Ham, Frank and You, Donghyun},
  booktitle={45th AIAA Aerospace Sciences Meeting and Exhibit},
  pages={1308},
  year={2007}
}

@article{amitay2001aerodynamic,
  title={Aerodynamic flow control over an unconventional airfoil using synthetic jet actuators},
  author={Amitay, Michael and Smith, Douglas R and Kibens, Valdis and Parekh, David E and Glezer, Ari},
  journal={AIAA journal},
  volume={39},
  number={3},
  pages={361--370},
  year={2001}
}

%*---Optimization
@article{duvigneau2006optimization,
  title={Optimization of a synthetic jet actuator for aerodynamic stall control},
  author={Duvigneau, R{\'e}gis and Visonneau, Michel},
  journal={Computers \& fluids},
  volume={35},
  number={6},
  pages={624--638},
  year={2006},
  publisher={Elsevier}
}
@article{duvigneau2006simulation,
  title={Simulation and optimization of stall control for an airfoil with a synthetic jet},
  author={Duvigneau, R{\'e}gis and Visonneau, Michel},
  journal={Aerospace Science and Technology},
  volume={10},
  number={4},
  pages={279--287},
  year={2006},
  publisher={Elsevier}
}



%*---SM
@article{jones2018controlexp,
  title={Control of flow separation around an airfoil at low Reynolds numbers using periodic surface morphing},
  author={Jones, G and Santer, M and Debiasi, M and Papadakis, G},
  journal={Journal of Fluids and Structures},
  volume={76},
  pages={536--557},
  year={2018},
  publisher={Elsevier}
}

@article{jones2018control,
  title={Control of low Reynolds number flow around an airfoil using periodic surface morphing: A numerical study},
  author={Jones, Gareth and Santer, Matthew and Papadakis, George},
  journal={Journal of Fluids and Structures},
  volume={76},
  pages={95--115},
  year={2018},
  publisher={Elsevier}
}

@article{akbarzadeh2020controlling,
  title={Controlling flow separation on a thick airfoil using backward traveling waves},
  author={Akbarzadeh, AM and Borazjani, I},
  journal={AIAA Journal},
  volume={58},
  number={9},
  pages={3799--3807},
  year={2020},
  publisher={American Institute of Aeronautics and Astronautics}
}

@inproceedings{akbarzadeh2019numerical,
  title={A numerical study on controlling flow separation via surface morphing in the form of backward traveling waves},
  author={Akbarzadeh, Amir and Borazjani, Iman},
  booktitle={AIAA Aviation 2019 Forum},
  pages={3589},
  year={2019}
}

@inproceedings{akbarzadeh2021role,
  title={The role of amplitude on controlling flow separation using traveling wave morphing},
  author={Akbarzadeh, Amir and Borazjani, Iman and Ogunka, Uchenna},
  booktitle={AIAA Scitech 2021 Forum},
  pages={2005},
  year={2021}
}

%*---Surface undualtions(fish)
@article{shukla2022hydrodynamics,
  title={Hydrodynamics study on a traveling wave-based undulating surface of a hydrofoil in a free-stream flow},
  author={Shukla, Sarvesh and Thekkethil, Namshad and Sharma, Atul and Agrawal, Amit and Bhardwaj, Rajneesh},
  journal={Physical Review Fluids},
  volume={7},
  number={8},
  pages={084703},
  year={2022},
  publisher={APS}
}

@article{akbarzadeh2019reducing,
  title={Reducing flow separation of an inclined plate via travelling waves},
  author={Akbarzadeh, AM and Borazjani, I},
  journal={Journal of Fluid Mechanics},
  volume={880},
  pages={831--863},
  year={2019},
  publisher={Cambridge University Press}
}

@article{thompson2022surface,
  title={Surface morphing for aerodynamic flows at low and stalled angles of attack},
  author={Thompson, Ernold and Goza, Andres},
  journal={Physical Review Fluids},
  volume={7},
  number={2},
  pages={024703},
  year={2022},
  publisher={APS}
}


@book{shyy2008aerodynamics,
  title={Aerodynamics of low Reynolds number flyers},
  author={Shyy, Wei and Lian, Yongsheng and Tang, Jian and Viieru, Dragos and Liu, Hao},
  year={2008}
}

@article{paris2023reinforcement,
  title={Reinforcement-learning-based actuator selection method for active flow control},
  author={Paris, Romain and Beneddine, Samir and Dandois, Julien},
  journal={Journal of Fluid Mechanics},
  volume={955},
  pages={A8},
  year={2023},
  publisher={Cambridge University Press}
}

@article{dickinson1993unsteady,
  title={Unsteady aerodynamic performance of model wings at low Reynolds numbers},
  author={Dickinson, Michael H and G{\"o}tz, Karl G},
  journal={Journal of experimental biology},
  volume={174},
  number={1},
  pages={45--64},
  year={1993},
  publisher={The Company of Biologists Ltd}
}

@article{flinois2015optimal,
  title={Optimal control of circular cylinder wakes using long control horizons},
  author={Flinois, Thibault LB and Colonius, Tim},
  journal={Physics of Fluids},
  volume={27},
  number={8},
  pages={087105},
  year={2015},
  publisher={AIP Publishing LLC}
}

@article{protas2002optimal,
  title={Optimal rotary control of the cylinder wake in the laminar regime},
  author={Protas, B and Styczek, Andrzej},
  journal={Physics of Fluids},
  volume={14},
  number={7},
  pages={2073--2087},
  year={2002},
  publisher={American Institute of Physics}
}

@article{naderi2016numerical,
  title={Numerical solution of unsteady flow on airfoils with local membrane in transient and laminar flows},
  author={Naderi, Alireza and Mojtahedpoor, Mohammad},
  journal={Journal of Theoretical and Applied Vibration and Acoustics},
  volume={2},
  number={1},
  pages={21--34},
  year={2016}
}

@article{jameson2003aerodynamic,
  title={Aerodynamic shape optimization using the adjoint method},
  author={Jameson, Antony},
  journal={Lectures at the Von Karman Institute, Brussels},
  year={2003}
}


@article{colonius2008fast,
  title={A fast immersed boundary method using a nullspace approach and multi-domain far-field boundary conditions},
  author={Colonius, Tim and Taira, Kunihiko},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={197},
  number={25-28},
  pages={2131--2146},
  year={2008},
  publisher={Elsevier}
}


@book{polak1971computational,
  title={Computational methods in optimization: a unified approach},
  author={Polak, Elijah},
  volume={77},
  year={1971},
  publisher={Academic press}
}

@book{press2007numerical,
  title={Numerical recipes 3rd edition: The art of scientific computing},
  author={Press, William H and Teukolsky, Saul A and Vetterling, William T and Flannery, Brian P},
  year={2007},
  publisher={Cambridge university press}
}

@article{bukshtynov2011optimal,
  title={On optimal reconstruction of constitutive relations},
  author={Bukshtynov, Vladislav and Volkov, Oleg and Protas, Bartosz},
  journal={Physica D: Nonlinear Phenomena},
  volume={240},
  number={16},
  pages={1228--1244},
  year={2011},
  publisher={Elsevier}
}

@article{kang2015effects,
  title={Effects of local oscillation of airfoil surface on lift enhancement at low Reynolds number},
  author={Kang, Wei and Lei, Pengfei and Zhang, Jiazhong and Xu, Min},
  journal={Journal of Fluids and Structures},
  volume={57},
  pages={49--65},
  year={2015},
  publisher={Elsevier}
}
@article{khan2017local,
  title={Local vibrations and lift performance of low Reynolds number airfoil},
  author={Khan, TariqAmin and Li, Wei and Zhang, Jiazhong and Shih, Tom IP},
  journal={Propulsion and Power Research},
  volume={6},
  number={2},
  pages={79--90},
  year={2017},
  publisher={Elsevier}
}

%*----

@inproceedings{thompson2023optimal,
  title={Optimal surface morphing using adjoint optimization},
  author={Thompson, Ernold and Goza, Andres},
  booktitle={AIAA SCITECH 2023 Forum},
  pages={0460},
  year={2023}
}



%% End of file `jfm2esam.bib'.

